PathFinder: Attention-Driven Dynamic Non-Line-of-Sight Tracking with a Mobile Robot

The study of non-line-of-sight (NLOS) imaging is growing due to its many potential applications, including rescue operations and pedestrian detection by self-driving cars. However, implementing NLOS imaging on a moving camera remains an open area of research. Existing NLOS imaging methods rely on time-resolved detectors and laser configurations that require precise optical alignment, making it difficult to deploy them in dynamic environments. This work proposes a data-driven approach to NLOS imaging, PathFinder, that can be used with a standard RGB camera mounted on a small, power-constrained mobile robot, such as an aerial drone. Our experimental pipeline is designed to accurately estimate the 2D trajectory of a person who moves in a Manhattan-world environment while remaining hidden from the camera's field-of-view. We introduce a novel approach to process a sequence of dynamic successive frames in a line-of-sight (LOS) video using an attention-based neural network that performs inference in real-time. The method also includes a preprocessing selection metric that analyzes images from a moving camera which contain multiple vertical planar surfaces, such as walls and building facades, and extracts planes that return maximum NLOS information. We validate the approach on in-the-wild scenes using a drone for video capture, thus demonstrating low-cost NLOS imaging in dynamic capture environments.

==> sec/2_relatedworks.tex <==
\section{Related Work}\label{sec:rw}
\paragraph{Passive %Non-line-of-Sight 
NLOS Imaging}
Passive  methods capture the visible light reflected from the hidden object to perform the NLOS imaging task. Due to the ill-posed nature of the problem, additional constraints and priors are often used for imaging, including partial occlusion~\cite{seidel2020two,torralba2014accidental}, polarization~\cite{yedidia2019using}, and coherence~\cite{beckus2019multi}.  Recently, the use of data-driven scene priors for passive NLOS imaging has shown great promise~\cite{tancik2018flash,aittala2019computational}. Tanick et al. used a CNN to perform activity recognition and tracking of humans and 
 a variational autoencoder to perform reconstructions~\cite{tancik2018flash}.  Sharma et al. proposed a deep learning technique that can detect the number of individuals and the activity performed by observing the LOS wall~\cite{sharma2021you}.  Wang et al. proposed a deep learning method that makes use of static and dynamic information about an NLOS scene to perform a tracking task~\cite{wang2023propagate}. They introduced the network PAC-Net, which alternately processes difference images and raw images to perform tracking. However, these methods are restricted to scenarios with a  static camera. 
 
 % \spr{(this is already said above) \sout{In this work, we propose a transformer architecture that can handle multiple surfaces present in a scene to predict the occluded object's position.}} % of the occluded object.

\paragraph{NLOS in Dynamic Scenarios}
There have been very few works dealing with the problem of NLOS with a moving detector.
Rabaste et al.~\cite{rabaste2017around} make use of a portable radar to detect and locate an NLOS object given a rough knowledge of the scene geometry. Scheiner et al.~\cite{scheiner2020seeing} explored the potential of Doppler radars for detection and tracking in dynamic settings. The authors depart from  visible-wavelength techniques and used indirect reflections for this purpose  and validated the method on in-the-wild automotive scenarios. 
% \sj{\sout{However, these approaches make use of radars in their setup.} \sout{Our goal with this work, however, is to propose a method that could work on consumer cameras that are already present on drones and robots, without the need to introduce additional acquisition modifications/setup.} }
% \spr{\sout{In this work, we propose a data-driven tracking network combined with a data-processing pipeline that allows us to demonstrate practical NLOS tracking in-the-wild using a simple consumer camera that can be mounted on a drone.}}

% \paragraph{\sj{\sout{NLOS Datasets}}}
% \sj{Comment: Let's just cite these two references when we introduce the datasets in 1 sentence, no need to devote a whole paragraph \sout{Galindo et al.~\cite{galindo2019dataset} published a dataset of synthetic time-resolved images of NLOS scenes targeted at benchmarking reconstructions. 
% Wang et al.~\cite{wang2023propagate} published a comprehensive passive NLOS dataset comprised of synthetic and real image data from environments with single blank planar walls. However, for our problem of dynamic NLOS imaging using a moving camera there is no readily available dataset with high-resolution ground truth trajectories. We believe the dataset captured for this work could greatly aid future NLOS works.} }
